Codebook Design for Composite Beamforming in Next-generation mmWave Systems

In pursuance of the unused spectrum in higher frequencies, millimeter wave (mmWave) bands have a pivotal role. However, the high path-loss and poor scattering associated with mmWave communications highlight the necessity of employing effective beamforming techniques. In order to efficiently search for the beam to serve a user and to jointly serve multiple users it is often required to use a composite beam which consists of multiple disjoint lobes. A composite beam covers multiple desired angular coverage intervals (ACIs) and ideally has maximum and uniform gain (smoothness) within each desired ACI, negligible gain (leakage) outside the desired ACIs, and sharp edges. We propose an algorithm for designing such ideal composite codebook by providing an analytical closed-form solution with low computational complexity. There is a fundamental trade-off between the gain, leakage and smoothness of the beams. Our design allows to achieve different values in such trade-off based on changing the design parameters. We highlight the shortcomings of the uniform linear arrays (ULAs) in building arbitrary composite beams. Consequently, we use a recently introduced twin-ULA (TULA) antenna structure to effectively resolve these inefficiencies. Numerical results are used to validate the theoretical findings.

==> L_free_formulation.tex <==
\section{New Formulation}
\label{new formulation}


\begin{align}
&\left(\mathbf{F}_{\text {opt }, q}, \mathbf{v}_{\mathrm{opt}, q}\right) \nonumber \\&=\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \int_{-\pi}^{\pi}\left|G_{\text {ideal }, q}(\psi)-G(\psi, \mathbf{F} \mathbf{v})\right|^{2} d \psi \nonumber \\
&= \underset{\mathbf{F}, \mathbf{v}}{\arg \min }\left[\lim _{L \rightarrow \infty} \sum_{p=1}^{2^{B}} \sum_{\ell=1}^{L} \frac{\left|G_{\text {ideal }, q}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \mathbf{F} \mathbf{v}\right)\right|^{2}}{L 2^{B} / 2 \pi}\right]\label{composite_MSE}
\end{align}


\begin{align}
\left(\mathbf{F}_{k}, \mathbf{v}_{k}\right) &=\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \sum_{p=1}^{2^{B}} \sum_{\ell=1}^{L}\left|G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \mathbf{F} \mathbf{v}\right)\right|^{2} \nonumber\\
&=\underset{\mathbf{F}, \mathbf{v}}{\arg \min }\frac{1}{L} \lim_{L\longrightarrow \infty}\left\|\mathbf{G}^L_{\text {ideal }, k}-\mathbf{G}(\mathbf{F} \mathbf{v})^L\right\|_{2}^{2} \label{init_opt}
\end{align}


where,  $$\mathbf{G^L}(\mathbf{F} \mathbf{v})=\left[G\left(\psi_{1,1}, \mathbf{F} \mathbf{v}\right) \cdots G\left(\psi_{2^{B}, L}, \mathbf{F} \mathbf{v}\right)\right]^{T} \in \mathbb{Z}^{L 2^{B}}$$

and, 
$$ \mathbf{G}^L_{\text {ideal }, k}=\left[G_{\text {ideal }, k}\left(\psi_{1,1}\right) \cdots G_{\text {ideal }, k}\left(\psi_{2^{B}, L}\right)\right]^{T} \in \mathbb{Z}^{L 2^{B}}$$

Note that it holds that 

\begin{equation}
    \mathbf{G}^L_{\text {ideal }, q}=\frac{2^{B}}{M_{t}}\left(\mathbf{e}_{q} \otimes \mathbf{1}_{L, 1}\right)
\end{equation}

For a suitable choice of $\g$ we can write: 
$$
\begin{aligned}
\mathbf{G}^L_{\text {ideal }, q} &=\frac{2^{B}}{M_{t}}\left(\mathbf{e}_{q} \otimes\left(\mathbf{g} \odot \mathbf{g}^{*}\right)\right) \\
&=\left(\sqrt{\frac{2^{B}}{M_{t}}}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right)\right) \odot\left(\sqrt{\frac{2^{B}}{M_{t}}}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right)\right)^{*}
\end{aligned}
$$

Similarly, we can write


\begin{align}
\mathbf{G}^L(\mathbf{F} \mathbf{v}) &=\left(\mathbf{D}^{L^H} \mathbf{F} \mathbf{v}\right) \odot\left(\mathbf{D}^{L^H} \mathbf{F} \mathbf{v}\right)^{*} \nonumber\\
\mathbf{D^L} &=\left[\mathbf{D^L}_{1} \cdots \mathbf{D^L}_{2^B} \right] \in \mathbb{C}^{M_{t} \times L 2^{\boldsymbol{B}}}
\end{align}

Given the last two equations, we can write, 

\begin{align}
&\left(\mathbf{F}_{\mid \mathbf{g}}, \mathbf{v}_{\mid \mathbf{g}}\right)=\nonumber\\
&\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \lim_{L\longrightarrow \infty} \frac{1}{L} \left\|\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)- \mathbf{D}^{H} \mathbf{F} \mathbf{v}\right\|_{2}^{2} \label{obj_func}\\
&\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \lim_{L\longrightarrow \infty} \frac{1}{L} \left\|\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)- \mathbf{D}^{H} \c_q \right\|_{2}^{2} \label{obj_func}
\end{align}

The last equation is a least square optimization problem.
 \begin{align}
& \c_q = (\D \D^H)^{-1} \D \gamma \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
& \c_q =  \gamma' \D \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
& \c_q =  \gamma' \D_q \mathbf{g}_q  
\end{align}

We aim to find $\g_q$ such that

\begin{align}
& \left\| abs(\D^H \gamma' \D_q \mathbf{g}_q)- abs(\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)) \right\|_{2}^{2}
\end{align}

We have

\begin{equation}
    c_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{j(m\psi_{q, l+1})} \quad \forall 0 \leq m \leq M_t-1
\end{equation}

With a choice of $\g = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ for $\alpha = e^j(\frac{2*\pi}{L2^B})$ and suitable $\eta$ (to be determined later), we can write


\begin{equation}
    c_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{2 \pi(\ell+0.5)}{L2^B})} \quad \forall 0 \leq m \leq M_t-1
\end{equation}


\begin{equation}
    c_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l} e^{jm(\psi_{q-1}+\frac{\pi}{L2^B})}  \quad \forall 0 \leq m \leq M_t-1
\end{equation}


\begin{equation}
    c_q^{(m)} = e^{jm(\psi_{q-1})}\lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l}   \quad \forall 0 \leq m \leq M_t-1
\end{equation}

\begin{equation}
    c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} \alpha^{(\eta + m)Lx}dx
\end{equation}


\begin{equation}
    c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\frac{2\pi(\eta + m)L}{L2^B}x}dx
\end{equation}


\begin{equation}
    c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\xi x}dx
\end{equation}

where $\xi = \frac{2\pi(\eta +m)}{2^B}$.


\begin{equation}
    c_q^{(m)} = e^{jm(\psi_{q-1})} \frac{e^{j\xi}-1}{j\xi}
\end{equation}

\begin{equation}
    c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} \frac{e^{j\xi/2}-e^{-j\xi/2}}{j\xi/2}
\end{equation}

\begin{equation}
    c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi})
\end{equation}

where $sinc(t) = \frac{sin(\pi t)}{\pi t}$.

==> alternative.tex <==
\section{Alternative Methods}
\label{sec:alternative}

Let's agree that equation (7) from \cite{love15} must hold, i.e.

\begin{equation}
    \alpha \mathbf{D}^{H} \mathbf{F} \mathbf{v}=\sqrt{\frac{2^{B}}{M_{t}}}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right) \label{eq7_paper}
\end{equation}
 
 Multiply both RHS and LHS by $D$ from left to get 
 
 \begin{equation}
     \alpha L \sqrt{\frac{2^B}{M_t}} \mathbf{Fv} = D_q \mathbf{g}
 \end{equation}
 
 Therefore, it is obvious that $\textbf{Fv} = \frac{D_q \textbf{g}}{\|D_q\textbf{g}\|}$ hs to be solved at some point. The challenge remains to find the suitable $\textbf{g}$ such that the gain  $G(\psi, \mathbf{c}) \doteq\left|\mathbf{d}_{M_{t}}^{H}(\psi) \mathbf{c}\right|^{2}$ remains close to the corresponding ideal gain. Maximizing $\|D_q\textbf{g}\|$ does not necessarily result in the desired property. We can write, 
 
 
 \begin{align}
     &D_q\mathbf{g} = \sum_{l=1}^{L}g_l\mathbf{d}_{M_t}(\psi_q, l)  \nonumber\\
     & = \sum_{l=1}^L g_l\left[{\begin{array}{cccc}
     1& e^{j\psi_{q, l}} &\cdots & e^{j(M_t-1)}\psi_{q, l}\\
     \end{array}}\right]^H \nonumber\\
     & = \left[{\begin{array}{cccc}
     \sum_{l=1}^L g_l& \sum_{l=1}^L g_le^{j\psi_{q, l}} &\cdots & \sum_{l=1}^L g_le^{j(M_t-1)\psi_{q, l}}\\
     \end{array}}\right]^H
 \end{align}
 
 Given that $\psi_{p, \ell}=\psi_{p-1}+\frac{2 \pi(\ell-0.5)}{L 2 ^B}$,  we can derive 
 
 \begin{equation}
 \c_q = \c_{q-1} \odot \left[{\begin{array}{cccc}
     1& \beta &\cdots & \beta^{M_t -1}
     \end{array}}\right]^H     
 \end{equation}

where $\beta = e^{j(\frac{2\pi}{2^B})}$. 
 
 Then we can write, 
 \begin{align}
     & \mathbf{d}_{M_{t}}^{H}(\psi) \mathbf{c_q}_{|\mathbf{g}} = 
     \sum_{l =1}^L{g_l(\sum_{m=0}^{M_t -1}}{e^{j(m(\psi_{q, l} -\psi))}})\nonumber\\
     & = \sum_{l =1}^L{\sum_{m=0}^{M_t -1}}{e^{j(\beta_l + m(\psi_{q, l} - \psi))}}
 \end{align}
 
 where $g_l =: e^{j\beta_l} $.
 
 \section{Least Square Solution}

The solution to the original optimization problem is \emph{equivalent} to the following optimization problem by introducing an auxiliary vector variable $\g$.
 
\begin{align}
&\left(\mathbf{F}_{\mid \mathbf{g}}, \mathbf{v}_{\mid \mathbf{g}}\right)=\nonumber\\
&\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \left\|\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)- \mathbf{D}^{H} \mathbf{F} \mathbf{v}\right\|_{2}^{2} \label{obj_func}\\
&\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \left\|\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)- \mathbf{D}^{H} \c_q \right\|_{2}^{2} \label{obj_func}
\end{align}

The last equation is a least square optimization problem.
 \begin{align}
& \c_q = (\D \D^H)^{-1} \D \gamma \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
& \c_q =  \gamma' \D \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
& \c_q =  \gamma' \D_q \mathbf{g}_q  
\end{align}

We aim to find $\g_q$ such that

\begin{align}
& \left\| abs(\D^H \gamma' \D_q \mathbf{g}_q)- abs(\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)) \right\|_{2}^{2}
\end{align}

is minimized.

Is it possible to show that $\g_q$ is independent of $q$ (assume regular scenario)? If true, i.e., $\g_q = \g$ we have

\begin{align}
     &D_q\mathbf{g} = \sum_{l=1}^{L}g_l\mathbf{d}_{M_t}(\psi_q, l)  \nonumber\\
     & = \sum_{l=1}^L g_l\left[{\begin{array}{cccc}
     1& e^{j\psi_{q, l}} &\cdots & e^{j(M_t-1)}\psi_{q, l}\\
     \end{array}}\right]^T \nonumber\\
     & = \left[{\begin{array}{cccc}
     \sum_{l=1}^L g_l& \sum_{l=1}^L g_le^{j\psi_{q, l}} &\cdots & \sum_{l=1}^L g_le^{j(M_t-1)\psi_{q, l}}\\
     \end{array}}\right]^T
 \end{align}
 
 Given that $\psi_{p, \ell}=\psi_{p-1}+\frac{2 \pi(\ell-0.5)}{L 2 ^B}$,  we can derive 
 
 \begin{equation}
 \c_q = \c_{q-1} \odot \left[{\begin{array}{cccc}
     1& \beta &\cdots & \beta^{M_t -1}
     \end{array}}\right]^T     
 \end{equation}

where $\beta = e^{j(\frac{2\pi}{2^B})}$. 
 
 Then we can write, 
 \begin{align}
     & \mathbf{d}_{M_{t}}^{H}(\psi) \mathbf{c_q}_{|\mathbf{g}} = 
     \sum_{l =1}^L{g_l(\sum_{m=0}^{M_t -1}}{e^{j(m(\psi_{q, l} -\psi))}})\nonumber\\
     & = \sum_{l =1}^L{\sum_{m=0}^{M_t -1}}{e^{j(\beta_l + m(\psi_{q, l} - \psi))}}
 \end{align}
 
 where $g_l =: e^{j\beta_l} $.
 
 A good choice for the vector $\g$ is $\g = \left[{\begin{array}{cccc} 1& \xi &\cdots & \xi^{L -1} \end{array}}\right]^T$ for some $\xi = \alpha^{\eta}$ where $\alpha = e^{j(\frac{ 2 \pi}{L2^B})}$.
 
The $k$-th entry of the vector $\c_q$, i.e., $\{\c_q\}_k$ in (\ref{}) can be written as follows when $L \longrightarrow \infty$. 
 \begin{align}
     & \sum_{l=1}^L g_le^{jk \psi_{q, l}} = \beta^{k} \frac{1}{L} \sum_{l=0}^{L-1} \alpha^{lk} g_l \\
     & = \beta^{k} \frac{1}{L} \sum_{l=0}^{L-1} \alpha^{lk} \alpha^{l \eta}  = \int_{0}^{1} \alpha^{(\eta+k)Lx} dx \\
     & = \int_{0}^{1} e^{j(\frac{ 2 \pi}{L2^B}) (\eta+k)Lx} dx \\
     & = \frac{e^{j \psi} - 1}{j \psi} = e^{\frac{j \psi}{2}} sinc(\frac{\psi}{2})
 \end{align}




==> derivation.tex <==
\section{Derivation}

In order to solve the above optimization problem, we write the 

\begin{align}
    \c_B^{opt} &= \underset{\c, \|\c\|=1}{\arg \min }\left[\lim _{L \rightarrow \infty} \frac{1}{L}\sum_{\ell=1}^{L} {\left|G_{\text {ideal }, B}\left(\psi_{ \ell}\right)-G\left(\psi_{\ell}, \c\right)\right|}\right]\label{composite_MSE}
\end{align}

 where, $\psi_{\ell} = -\pi + \ell(\frac{2\pi}{L})$. We can rewrite equation \eqref{composite_MSE} as follows, 

\begin{align}
 &\c_B^{opt} = \underset{\c,  \|\c\|=1}{\arg \min } \lim_{L\rightarrow \infty}\frac{1}{L}|\mathbf{G}_{\text {ideal }, k}-\mathbf{G}(\c)| \label{init_opt}
 \end{align}
 
 where,  $$\mathbf{G}(\c)=\left[ G\left(\psi_{1}, \c\right) \ldots G\left(\psi_{L}, \c\right)\right]^{T} \in \mathbb{Z}^{L}$$

and, 
$$ \mathbf{G}_{\text {ideal }, B}=\left[ G_{\text {ideal }, B}\left(\psi_{1}\right) \ldots G_{\text {ideal }, B}\left(\psi_{ L}\right)\right]^{T} \in \mathbb{Z}^{L}$$


Note that it holds that 

\begin{equation}
    \mathbf{G}_{\text {ideal },B}=\sum_{s =1}^{S/2}\frac{2\pi}{\Delta_B}\left(\mathbf{e}_{s} \otimes \mathbf{1}_{L_s, 1}\right) \label{ideal}
\end{equation}

with $\mathbf{e}_{s} \in \mathbb{Z}^{S}$ being the standard basis vector for the $s$-th axis among $S$ ones. Now, note that $\mathbf{1}_{L_s, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any equal gain $\mathbf{g} \in \mathbb{C}^{L_s}$. Therefore, for such choice of $\g$ we can write: 

% $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$


\begin{align}
\mathbf{G}_{\text {ideal }, B} &= \sum_{s=1}^{S/2}\frac{2\pi}{\Delta_B}\left(\mathbf{e}_{s} \otimes\left(\mathbf{g}_s \odot \mathbf{g}_s^{*}\right)\right) \nonumber\\
&=\sum_{s =1}^{S/2}\left({\gamma_s}\left(\mathbf{e}_{s} \otimes \mathbf{g}_s\right)\right) \odot\left({{\gamma_s}}\left(\mathbf{e}_{s} \otimes \mathbf{g}_s\right)\right)^{*} \nonumber\\
&=\left(\sum_{s =1}^{S/2}{\gamma_s}\left(\mathbf{e}_{s} \otimes \mathbf{g}_s\right)\right)  \odot \left(\sum_{s=1}^{S/2}{\gamma_s}\left(\mathbf{e}_{s} \otimes \mathbf{g}_s\right)\right)^{*} \label{final_gik}
\end{align}

Similarly, it is straightforward to observe,


\begin{align}
\mathbf{G}(\c) &=\left(\mathbf{D}^{H} \c\right) \odot\left(\mathbf{D}^{H} \c\right)^{*} \label{dc}
\end{align}
where $\mathbf{D} =\left[\mathbf{D}_{1}, \cdots, \mathbf{D}_{S} \right] \in \mathbb{C}^{M_{t} \times L}$, and for $s=1, \cdots, S$
$\mathbf{D}_{s}=\left[\mathbf{d}_{M_{t}}\left(\psi_{s, 1}\right) \cdots \mathbf{d}_{M_{t}}\left(\psi_{s, L_s}\right)\right] \in \mathbb{C}^{M_{t} \times L_s}.$

Comparing the expressions \eqref{init_opt}, \eqref{final_gik}, and \eqref{dc}, one can show that the optimal choice of $\c^{opt}_B$ in \eqref{init_opt} is the solution to the following optimization problem for proper choices of $\g_s$. 
\begin{problem}
Given equal-gain vectors $\g_s \in \mathbb{C}^{L_s}$, $s =1, \cdots, S/2$, find vector $\c_B \in \mathbb{C}^{M_t}$ such that
\begin{align}
&\c_B=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\rightarrow \infty} \left\|\sum_{s=1}^{S/2}{\gamma_s}\left(\mathbf{e}_{s} \otimes \mathbf{g}_s\right)- \mathbf{D}^{H} \c\right\|^{2} \label{obj_func}
\end{align}
\label{main_problem}
\end{problem}


However, we now need to find the optimal choices for $\g_s$ that minimize the objective in \eqref{init_opt}. Using \eqref{final_gik}, and \eqref{dc}, we have the following optimization problem.
\begin{problem}
Find a set of equal-gain $\g_s \in \mathbb{C}^{L_s}$, i.e. $\mathcal{G}_B$ such that
\begin{equation}
 \mathcal{G}_B = \underset{\mathcal{G}}{\arg\min }\left\| abs(\D^H \c_B)- abs(\sum_{s=1}^{S/2}{\gamma_s}(\mathbf{e}_{s} \otimes \mathbf{g}_s))\right\|^{2} \label{g_final_eq}
\end{equation} 
where $\mathcal{G}_B = \{\g_s| s= 1, \cdots, S/2\}$, and $abs(.)$ denotes the element-wise absolute value of a vector.
\label{g_problem}
\end{problem}

Hence, the codebook design for a system with fully-digital beamforming capability is found by solving Problem~\ref{main_problem} for proper choices of $\g_s$ obtained as a solution to Problem ~\ref{g_problem}. The codebook for Hybrid beamforming, is then found as
\begin{align}
    \mathbf{F}_{B}, \mathbf{v}_{B} = \underset{\mathbf{F},\mathbf{v}}{\arg\min } \|\mathbf{F}\mathbf{v} - \c^{opt}_B\|^2
\end{align}
where the columns of $\F_B \in \mathbb{C}^{M_t \times N_{RF}}$ are equal-gain vectors and $\v_B \in \mathbb{C}^{N_{RF}}$. The solution may be obtained using simple, yet effective suboptimal algorithm such as orthogonal matching pursuit (OMP) \cite{love15}\cite{noh17}\cite{Hussain17}. In the next section we continue with the solution of Problem~\ref{main_problem}, and~\ref{g_problem}.


Note that the solution to problem \ref{main_problem} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity. For each $L$ we find that,
 \begin{align}
& {\c}^{(L)}_B = \sum_{s =1}^{S/2}{\gamma_s}(\D \D^H)^{-1} \D  \left(\mathbf{e}_s \otimes \mathbf{g}_s\right) \\
& {\c}^{(L)}_B = \sum_{s=1}^{S/2}\sigma_s \D_s\g_s \label{c_final_eq}
\end{align}
where $\sigma_s = \frac{\gamma_s}{L} = \frac{\sqrt{\frac{2\pi}{\Delta_B}}}{L}$, noting that it holds that, 

$$\mathbf{D D}^{H}  = \sum_{s=1}^S \D_s{ \D}_s^{H} = \sum_{s=1}^S L_s\I_{M_t} = L\I_{M_t}$$
% $$\mathbf{D D}^{H}=\left({L \sum_{p=1}^{2^B}\delta_p}\right) \mathbf{I}_{M_{t}}$$.
% % Dividing by $\|\Tilde{\c}^{(L)}_q\|$ and taking the limit as L goes to infinity we will find the optimal $\c_q$. i.e. 


Using \eqref{c_final_eq}, equation \eqref{g_final_eq} can now be rewritten as, 

\begin{align}
 &\mathcal{G}_B = \underset{\mathcal{G}}{\arg\min } \nonumber
 \\&\left\| abs(\D^H \D\sum_{s=1}^{S/2}\sigma_s(\mathbf{e}_{s} \otimes \mathbf{g}_s))-abs(\sum_{s=1}^{S/2}{\gamma_s}(\mathbf{e}_{s} \otimes \mathbf{g}_s))\right\|^{2} \label{g_simple_final_eq}
\end{align} 

% where $\sigma' = \frac{1}{2\pi L}$. We will state the following theorem without formal proof.
\begin{proposition}
The minimizer of \eqref{g_simple_final_eq} is in the form of geometric vectors $\g_s = \g_{L_s}(\frac{\eta\delta_s}{L})$, $s=1 \cdots S$ for some real value $\eta\geq 0$. \label{proposiiton_g}
\end{proposition}

An analytical closed-form solution for $\c_B$ can be found as follows. We have, 
 \begin{align}
     {\c_B}^{(L)} & = \sum_{s =1}^{S/2} \sigma_s \left(\sum_{l=1}^{L_s}g_{s, l}\mathbf{d}_{M_t}(\psi_{s, l})\right)  \nonumber\\
     & = \sum_{s=1}^{S/2} \left(\sum_{l=1}^{L_s} \sigma_sg_s^{(l)}\left[{\begin{array}{ccc}
     1 &\cdots & e^{j(M_t-1)\psi_{s, l}}\\
     \end{array}}\right]^T \right)  
    %  & = \sum_{q \in \mathcal{W}_k} \sigma_q \left[{\begin{array}{ccc}
    %  \sum_{l=1}^L g_{q, l}& \cdots & \sum_{l=1}^L g_{q, l}e^{j(M_t-1)\psi_{q, l}}\\
    %  \end{array}}\right]^T 
\end{align}

 
% Let us write, 

% \begin{equation}
%     \c_k^{(L)} = \sum_{q \in \mathcal{W}_k} \c_q^{(L)}
% \end{equation}

Define, 

\begin{equation}
{\c_s}^{(L)}  = \sigma_s \sum_{l=1}^{L_s}g_{s, l}\mathbf{d}_{M_t}(\psi_{s, l})
\end{equation}

to get,

\begin{equation}
    \c_B^{(L)} = \sum_{s=1}^{S/2} \c_s^{(L)}
\end{equation}


The $m$-th element of the vector ${\c}_s = \lim_{L\rightarrow \infty}{\c_s}^{(L)} $, i.e. $c_{s,m}$, is given by 

\begin{align}
    c_{s,m} &= \sqrt{\frac{2\pi}{\Delta_B}}\lim_{L\rightarrow \infty} \frac{1}{L}\sum_{l=0}^{L_s-1} g_{s, l} e^{jm\psi_{s, l}} \nonumber\\
    & = \frac{\delta_s}{\sqrt{ 2\pi\Delta_B}}\lim_{L_s\rightarrow \infty} \frac{1}{L_s}\sum_{l=0}^{L_s-1} g_{s, l} e^{jm\psi_{s, l}}
\end{align}

% With a choice of $\g_q = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ where we set 
% % $\alpha = e^j(\frac{2\pi}{L2^B})$
% $\alpha = e^{j(\frac{\delta_q}{L})}$ and suitable $\eta$ (to be determined later), we can write


% \begin{equation}
%     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{2 \pi(\ell+0.5)}{L2^B})}
% \end{equation}

Choosing $\g_b$ as in proposition \ref{proposiiton_g}, and replacing $\psi_{b,l} = \psi_b^s + l\frac{\delta_b}{L_b}$

\begin{align}
    c_{b,m} &= \frac{\delta_b}{\sqrt{ 2\pi\Delta_B}}\lim_{L_b\rightarrow \infty} \frac{1}{L_b}\sum_{l=0}^{L_b-1} e^{j\frac{l\eta\delta_b}{L_b}} e^{jm(\psi_b^s + l\frac{\delta_b}{L_b})} \nonumber \\
    &= \frac{\delta_b}{\sqrt{ 2\pi\Delta_B}}e^{jm(\psi^s_{b})}\lim_{L\rightarrow \infty} \frac{1}{L_b}\sum_{l=0}^{L_b-1} \alpha^{(\eta+m) l}   \nonumber \\
    &= \frac{\delta_b}{\sqrt{ 2\pi\Delta_B}}e^{jm(\psi^s_{b})} \int_{0}^{1} \alpha^{(\eta + m)L_bx}dx
\end{align}

\noindent where $\alpha = e^{j\frac{\delta_b}{L_b}}$. After a few straightforward steps, we get,  

% \begin{equation}
%     c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}\lim_{L\rightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_{q, l} e^{jm(\psi_{q-1}+\frac{\delta_q(\ell+0.5)}{L})}
% \end{equation}

% % After some basic manipulations we get, 
% \begin{equation}
%     c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}\lim_{L\rightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l} e^{jm(\psi_{q-1}+\frac{0.5\delta_q}{L})} 
% \end{equation}


% \begin{equation}
%     c_{b,m} = \frac{\delta_b}{\sqrt{ 2\pi\Delta_B}}e^{jm(\psi^s_{b})}\lim_{L\rightarrow \infty} \frac{1}{L_b}\sum_{l=0}^{L_b-1} \alpha^{(\eta+m) l}   
% \end{equation}

% \begin{equation}
%     c_{b,m} = \frac{\delta_b}{\sqrt{ 2\pi\Delta_B}}e^{jm(\psi^s_{b})} \int_{0}^{1} \alpha^{(\eta + m)L_bx}dx
% \end{equation}


% \begin{equation}
%     c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\frac{2\pi(\eta + m)L}{L2^B}x}dx
% \end{equation}


\begin{align}
 c_{b,m}= \frac{\delta_b}{\sqrt{ 2\pi\Delta_B}}e^{j(m\psi^s_{b} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi}) \label{final_g}
\end{align}

where $\xi = \delta_b (\eta +m )$.


==> introduction1.tex <==
\section{Introduction}





%%-------Abstract of Related work--------%%

Obtaining accurate CSI is essential for effective beamforming in MIMO systems, however, due to the large number of antennas at mmWave band, this information is hardly available. Some works mainly focus on the channel estimation problem either by using feedback from the receiver \cite{khateeb14}\cite{noh16}\cite{noh17}, or by using prior assumptions on the channel statistics such as the channel covariance matrix, its sparsity, low rank, etc. \cite{song15}\cite{vlachos18}\cite{vlachos19}. To relax the channel estimation challenges, a line of research suggests to employ a hierarchical multi-level beamforming and codebook design, where the AoD/AoA interval is split into disjoint regions and is searched sequentially at increasing resolution using multi-level codebooks and sounding the corresponding beamformers \cite{noh17}\cite{love15}\cite{qiao17}. The beam search problem is modeled and solved in \cite{noh17}\cite{Hussain17} as a Neyman-Pearson (NP) detection problem with the objectives of maximizing the data rate and spectral efficiency, while the authors in \cite{noh17} propose a DFT-based hybrid codebook design by the objective of minimizing the gain variance at main lobe, and the authors in \cite{love15}\cite{{song15}} aim at minimizing the distance of the designed gain from the ideal one. Once the codebook for digital beamforming is designed, a simple but yet effective OMP algorithm is used to construct the near-optimal hybrid beamformers. 
More recently, another line of work has started efforts in employing machine learning based methods for channel estimation and hybrid beamforming in MIMO systems \cite{Tao}\cite{Elbir}\cite{Coleri}\cite{chen}. 









---Beam alignment techniques for mmWave relies on beams that are covering
 
5th generation of wireless cellular communication systems relies on millimeter Wave (mmWave) frequencies as a key enabler to realize one of its key promises, i.e. enhanced mobile broadband (eMBB). This is due to Gigahertz of bandwidth available beyond $20$ GHz frequency range. However, due to the severe path-loss and poor scattering associated with mmWave frequency bands, effective beamforming techniques employing massive MIMO systems are essential to deal with such difficulties. 

Given the large number of antennas in such systems, it may not be cost/power-efficient to deploy one radio-frequency (RF) chain per antenna, therefore, traditional \emph{fully digital} beamforming approaches may not be feasible. Instead, it is preferred to employ a few phase-shifters in conjunction with baseband beamformers that are in charge of adjusting the gain of the signals input to each RF chain. This approach known as \emph{hybrid} beamforming has been extensively used  in the literature to design effective beamformers. %Need to input the citations here

Given the large size of the channel due to the large number of antennas, estimating the channel state information (CSI) at the receiver is cumbersome, therefore, the transmitter has to rely on feedback from the receiver on the quality of received signal. Within the beamforming procedure, a codebook is utilized that is known to both the transmitter and the receiver. The codebook consists of a number codewords (beamforming vectors), each tailored to a transmit beam. At the end of the feedback-based beam search procedure, the receiver will have chosen the suitable beamforming vector from the codebook. There is a trade-off associated with the sharp narrow beams, and the complexity of the feedback-based beam search procedure. 

In this paper, we study the codebook design problem considering both the digital and hybrid beamforming approaches. Under the fully digital scheme, We first consider a uniform linear array (ULA) of antennas and design the codebook to minimize the mean-square error (MSE) between the desired ideal beam gain and the beam gain resulted from the designed beamforming vector. We next use the orthogonal matching pursuit (OMP) algorithm to design near-optimal baseband and analog beamforming vectors based on the designed codeword for each beam to complete the design of the hybrid beamforming method. In contrast to the methods described in \cite{love15}, and \cite{song15} that utilize the quantization of the angular space, we output a closed-form for the designed codebook that does not rely on such quantization. Moreover, the gain of the designed beams under the ULA structure, is symmetric with respect to the origin of the angular space, by the definition. In other words, the designed codewords create two main-lobes one of which is redundant. This will result in a significant design suboptimality and generates a lower gain within the desired main lobe. To deal with this issue, we introduce a new structure of antennas, namely, \emph{twin} ULA (TULA) which consists of two ULAs that are placed in th 2D plane parallel to each other along one axis and with a fixed distance along the other axis. We show that our new design under this setting allows not only suppresses the undesired beams, but also improves the gain of the desired main lobe. 

The contributions of this paper are as follows:
\begin{itemize}
\item We introduce Twin ULA (TULA) that is novel antenna configuration. TULA is different from UPA in the following senses: (1) TULA is not uniform (2) the plane of UPA is orthogonal to the azimuth plane while the plane of TULA is the azimuth plane.

\item We drive low-complexity analytical solution for the optimal beams for ULA, TULA, delta, and star configuration. This analytical solution eliminates the need for an exhaustive search in finding the optimal beams \cite{love15}\cite{song15}. The solution to hybrid beamforming when the second beamforming stage is a  

\end{itemize}

%This is completely copied from the other paper. Need to refine and rephrase.
\textbf{Notation} Throughout this paper, $\mathbb{C}$ denotes the set of complex numbers, $\mathcal{C N}\left(m, \sigma^{2}\right)$ denotes the complex normal distribution with mean $m$ and variance $\sigma^{2}$, $[a, b]$ is the closed interval between $a$ and $b, \mathbf{1}_{a, b}$ is the $a \times b$ all ones matrix, $\mathbf{I}_{N}$ is the $N \times N$ identity matrix, is the ceiling function, $\mathds{1}_{[a, b)}$ is the indicator function, $\|\cdot\|$ is the $2$ -norm, $\odot$ is the Hadamard product, $\otimes$ is the Kronecker product, $\mathbf{A}^{H},$ and $\mathbf{A}_{a, b}$ denote conjugate transpose, and $(a, b)^{t h}$ entry of \A respectively.





The remainder of the paper is organized as follows. Section~\ref{sec:desc} describes the system model. In Section~\ref{sec: formulation} we formulate the codebook design problem and propose our solutions in section ~\ref{sec: proposed}. Section ~\ref{sec:evaluation} presents our evaluation results, and finally, in Section ~\ref{sec:conclusions}, we highlight our conclusions and discuss directions for future work.


==> related_work.tex <==
\section{Related Work}
\label{sec: related}

Considerable amount of research has been allocated in the literature to the design of mmWave MIMO systems and optimizing the beamforming schemes. Given the importance of accurate CSI which is hardly available due to the large scale of the system, in beamforming training, some works focus on the channel estimation problem as their main theme either using feedback from the receiver \cite{khateeb14}\cite{noh16}\cite{noh17}, or by using the prior assumptions on channel statistics, such as its covariance matrix, sparsity, low rank, etc. \cite{song15}\cite{vlachos18}\cite{vlachos19}.

To deal with the channel estimation challenges, a line of research has been dedicated to the hierarchical multi-level beamforming and codebook design, where the AoD/AoA interval is split into disjoint regions and is searched sequentially at increasing resolution using multi-level codebooks and sounding the corresponding beamformers \cite{noh17}\cite{love15}\cite{qiao17}. 

In \cite{ayach14}, the authors aim at improving the MmWave spectral efficiency via beamforming with multiple data streams, where they consider both the transmitter precoding and the receiver combining problems given hardware constraints. They formulate the precoding problem as the maximization of the mutual information between the baseband and the RF precoders, subject to transmitter's total power and RF precoder constant gain constraints. Given the near-optimal precoder the combining problem at the receiver is formulated as an MMSE optimization problem to minimize the error of the reconstruction of the transmitted signal. The approach for solving the two models is based on the OMP algorithm utilizing the array response vector as the columns of the approximate solution. 

In \cite{song15}, a soft beam alignment algorithm is proposed based on multiple channel soundings that are performed using different training beamforming vectors and observing the outputs under dual-polarized antenna regime. The authors first focus on optimizing the channel gain under perfect channel knowledge. They will then remove perfect CSI assumption and show that it is not possible to perform a hard beam alignment decision at low SNR due to the difficulty in channel estimation  under high-variance noise. They show that adaptively increasing the number of training vectors does not mitigate this issue. They next propose an MLE approach for estimating the channel parameters based on the observed outputs and show how effectively their approach addresses the above-mentioned problems. 

The work in \cite{noh17} considers two related problems. The authors first propose a multi-level beamforming framework via an iterative algorithm for beam-searching given a pre-defined set of codebooks. The receiver employs a Neyman-Pearson (NP) rule to detect the beam over which the received signal strength is above a given threshold within a desired sector, and the transmitter aims at striking a balance between the achievable data rate and the training overhead. In the second phase, a hybrid beamforming structure is considered where the authors propose a DFT-based codebook design method and aim at minimizing the variance of the achieved gain within the corresponding lobe to reach the desired constant main lobe gain.

The authors in \cite{Hussain17}, propose a codebook design method based on the NP decision rule, assuming that the the desired range of AoD is already computed and given as input to the decision problem. The codeword should be designed in a way that the receiver can decide between AoD being within the given range or not; i.e. the codeword should be designed such that the misdetection probability is minimized given that the false alarm probability is upper-bounded. The authors formulate such optimization problem and come up with a near-optimal solution for the codeword. Next, they employ the OMP algorithm to find the values for the analog and digital precoder in the hybrid beamforming regime. 


==> story.tex <==

%------------------------storyline
State of the art design: 

We focus a codebook design scenario where the whole azimuth angle of $2\pi$ is uniformly split to equal beam-widths each of which is excited by one of the codewords. Figure 1 efgh shows the codebook design in [10] which achieves equal beamwidths. This figures were regenerated based on the design in [10] using L=300 and all ones vector for g. Using the same antenna configuration (ULA), Fig 1 abcd shows our design which improves on the design in [10] in terms of the gain by choosing optimal g. Further, the form of the optimal g is derived and optimized with very low computational complexity. Both design in [10] and our design generate beams with fairly sharp edges and have relatively stable gain in the coverage area.

(gain improvement by reflecting the beams)

However, the design in Fig a-h suffers from multiple shortcomings. (a) First, due to the behavior of ULA any beam is symmetrical with respect to the ULA axis (i.e., the line passing through the base of the antennas). This means that any beams designed using ULA is two-sided, e.g., the beams which covers 22.5-45deg will cover the -22.5 to -45deg as well. (b) Second, the gains of the beams covering different arcs vary considerably. (c) Third, the beams that are close to the direction of the antennas are neither so sharp nor have stable gains.

Fig 1 ijkl is the regeneration of the design in [1] which attempts to generated beams that have almost equal gain for all arcs. Please note that these figures are generated by using the analytical optimal g rather than searching over a large predefined set as in [1]. Even though the variation in the gain of the beams across different beams may be controlled by using design in [1], this design is not following the initial condition of having uniform beam-widths, hence it is not appropriate design when such uniform beamwidth is required. Indeed, the reason behind having similar gains across different arcs may be explained by the scaling factor which is equal to the beamwidths and affects the beam power: The gains of the beams are increased by decreasing their beamwidth as in (equation number).

In order to overcome shortcoming (a), we present a novel idea of Twin ULA (TULA). Fig2. ab illustrates the first 8 beams of a codebook with 16 beamforming vectors. It can be seen that TULA is very effective to generate one-sided beams. Fig.2 ef illustrates all 16 beams of the same codebook. It is observed that not only TULA solves shortcoming (a) but also it provides considerable gain improvement (almost double). This can be interpreted as removing the unwanted signal in the unwanted angular interval on the other side of the antenna axis and contributing to the desired angular interval. Nonetheless, the shortcoming (b) and (c) are still outstanding in TULA design.

Please note that our framework for the design of TULA allows to use similar design as in [1] in order to have comparable gains across all beams as illustrated in Fig2 cd. However, as mentioned before, such design is not following the initial condition of having uniform beam-widths across all beams.

Fig1. bdfhjl and Fig2.gh show the hybrid beamforming design for NRF=4 of the corresponding Fig.acegik and Fig2.ef, respectively. It can be seen that with the codebook size of up to 16 the loss of using hybrid beamforming instead of Fully digital beamforming is not noticeable.

In order to address the shortcomming (b) and (c), we propose two more antenna configurations: Delta ($\Delta$) and Star.
Fig.5 and 6 illustrates the beam patterns of a codebook of size 6 using Delta configuration. Fig.7 and 8 illustrates the beam patterns of a codebook of size 12 and fig 9 shows the beam pattern of a codebook of size 24 using Delta configuration.
It is observed that the beam patterns have relatively sharp edges, almost similar gain across the beams, relatively constant gain over the beamwidth, and precisely splitting the azimuth angle into equal size beamwidths. 

Finally, Fig 3 and 4 illustrates the beam patterns of a codebook of size 16 using star configuration. It is understood that as the number of beams in the codebook increases, the sharpness of the beams decreases and in order to design the beams with the same sharpness, the number of antennas has to increase.

%---------------------
